Robust Scheduling with GFlowNets

Finding the best way to schedule operations in a computation graph is a classical NP-hard problem which is central to compiler optimization. However, evaluating the goodness of a schedule on the target hardware can be very time-consuming. Traditional approaches as well as previous machine learning ones typically optimize proxy metrics, which are fast to evaluate but can lead to bad schedules when tested on the target hardware. In this work, we propose a new approach to scheduling by sampling proportionally to the proxy metric using a novel GFlowNet method. We introduce a technique to control the trade-off between diversity and goodness of the proposed schedules at inference time and demonstrate empirically that the pure optimization baselines can lead to subpar performance with respect to our approach when tested on a target model. Furthermore, we show that conditioning the GFlowNet on the computation graph enables generalization to unseen scheduling problems for both synthetic and real-world compiler datasets.

==> sections/6_Proof_old.tex <==
\section{Proof for Theorem 1}
\label{prf:rew_continuity}
In the following, we will denote $F^R$ to be the flow corresponding to a flow function $F: \mathcal{T}\rightarrow \mathbb{R}_{\geq 0}$ with corresponding reward $R$.
That is, $F^R : \mathcal{T} \rightarrow \mathbb{R}_{\geq 0}$ is a flow function such that for any terminal state $\scdl$ we have $R(\scdl)=\sum_{\trj\in\mathcal{T}_\scdl}F^R(\trj)$, where $\sum_{\trj\in\mathcal{T}_\scdl}F^R(\trj)\eqqcolon F^R(\scdl)$ is the total flow at the terminal state $\scdl$.

% In the following, we denote the total flow at the terminal state $\scdl$ as $F^R(\scdl):=\sum_{\trj\in\mathcal{T}_\scdl}F(\trj)$.
% That is, $F^R : \mathcal{T} \rightarrow \mathbb{R}^+$ is a flow function, such that for any terminal state $x \in S$ we have $F^R(x) = R(x)$, where $F(s') = \sum_{s\rightarrow s' \in \tau} F(\tau)$ is the sum of trajectory flow values over trajectories containing the transition from an arbitrary state $s$ into $s'$.

%\begin{lemma}[Flow Decomposition]
%\label{lemma:decomp}
%For all reward functions $R_1 \geq 0, R_2 \geq 0$ such that $R_1+R_2 = R$ and for all corresponding flow functions $F^R$, there exist flow functions $F^{R_1}, F^{R_2}$ such that $F^{R_1} + F^{R_2} = F^{R}$. 
%\end{lemma}

%\textit{Proof.} We will start by constructing $F^{R_1}$ to be a flow that results from reducing the edge flow of $F^R$ accordingly. Let $\{x_i\}_{i=1}^M$ be the set of terminal states and define

%\begin{equation}
%F^{R_1}(\tau) :=
%        \sum_{i=1}^M \mathds{1}_{x_i\in\tau} \left(\frac{R_1(x_i)}{R(x_i)}F^R(\tau)\right)
%\end{equation}

%Then, for any terminal state $x$, we have

%\begin{equation}
%    F^{R_1}(x) = \sum_{\tau: x\in\tau}F^{R_1}(\tau) = \sum_{\tau: x\in\tau} \frac{R_1(x)}{R(x)}F^R(\tau) =  \frac{R_1(x)}{R(x)} \sum_{\tau: x\in\tau}F^R(\tau) = R_1(x),
%\end{equation}

%thus yielding a flow function for $R_1$. For $R_2$, simply define $F^{R_2} := F^R-F^{R_1}$. By construction of $F^{R_1}$, $F^{R_2}(\tau) \geq 0$ for all $\tau$ and, by definition, $F^{R_2}(x) = R_2(x)$ follows.

\begin{theorem*}[Flow Continuity]
    Let $\{R_i\}_{i=1}^\infty$ be a sequence of positive reward functions such that for all terminal states $x$, $(R_i(x)/R(x)) \rightarrow 1$ as $i \rightarrow \infty$. Then, for any flow $F^R$ with reward $R$, there exists a sequence of flow functions $\{F^{R_i}\}_{i=1}^\infty$ with $F^{R_i}(\trj) \rightarrow F^R(\trj)$ for all $\trj \in \mathcal{T}$.
\end{theorem*}

%\textit{Proof.} Let $\epsilon >0$, $\tau \in \mathcal{T}$ be arbitrary with terminal state $x$ and choose $N_0 \in \mathbb{N}$ such that $(R_i(x)-R(x)) < \epsilon$ for all $i \geq N_0$. By lemma \ref{lemma:decomp}, we can decompose $F^{R_i}$ into $F^{R} + F^{R_i-R}$. Now, for all $i\geq N_0$ we have $F^{R_i-R}(\tau) \leq F^{R_i-R}(x) = R_i(x)-R(x) < \epsilon$ and hence $F^{R_i}(\tau) \rightarrow F^{R}(\tau)$.

%\textit{Proof.} We will start by constructing a sequence $\{F^{R_i+R}\}_{i=1}^\infty$ from $F^{R}$. Let $\{x_i\}_{i=1}^M$ be the set of terminal states and define 

%\begin{equation}
%F^{R_i+R}(\tau) :=
%        \sum_{k=1}^M \mathds{1}_{x_k\in\tau} F^R(\tau) \left(1 + \frac{R_i(x_k)}{R(x_k)}\right).
%\end{equation}

%To see that $F^{R_i+R}$ is a valid flow for $R_i+R$, we note that $F^{R_i+R} \geq 0$ and

%\begin{align}
%\begin{split}
%    F^{R_i+R}(x) &= \sum_{\tau: x\in\tau}F^{R_i+R}(\tau) = \left(1 + \frac{R_i(x)}{R(x)}\right) \sum_{\tau: x\in\tau}F^R(\tau) \\
%    &=  \left(1 + \frac{R_i(x)}{R(x)}\right) R(x) = R_i(x)+R(x)
%\end{split}
%\end{align}

%for any terminal state $x \in S$. Now, by construction, $F^{R_i} := F^{R_i+R}-F^{R}$ is a well defined flow for $R_i$ since $F^{R_i+R} \geq F^R$ and $F^{R_i}(x) = F^{R_i+R}(x) - F^R(x) = R_i(x)$. Finally, we see that for any $\tau \in \mathcal{T}$ with terminal state $x$

%\begin{equation}
%    F^{R_i}(\tau) =  \left(1 + \frac{R_i(x)}{R(x)}\right)F^{R}(\tau) - F^{R}(\tau) = \frac{R_i(x)}{R(x)}F^R(\tau) \rightarrow F^R(\tau).
%\end{equation} \hfill $\blacksquare$

\textit{Proof.} Let $\{x_i\}_{i=1}^M$ be the set of terminal states and define 

\begin{equation}
F^{R_i}(\trj=(s_0, \dots,\scdl)) \coloneqq F^R(\trj) \frac{R_i(x)}{R(x)}
\end{equation}

To see that $F^{R_i}$ is a valid flow for $R_i$, we note that $F^{R_i} \geq 0$ and

\begin{align}
\begin{split}
    F^{R_i}(\scdl)&=\sum_{\trj\in\mathcal{T}_{\scdl}}F^{R_i}(\trj) = \frac{R_i(x)}{R(x)} \sum_{\trj\in\mathcal{T}_{\scdl}}F^R(\trj) \\
    &=  \frac{R_i(x)}{R(x)} R(x) = R_i(x)
\end{split}
\end{align}

for any terminal state $\scdl$. Finally, for any $\trj \in \mathcal{T}$ with terminal state $\scdl$ we have

\begin{equation}
    F^{R_i}(\trj) =  \frac{R_i(\scdl)}{R(\scdl)}F^{R}(\trj)  \rightarrow F^R(\trj)
\end{equation} \hfill $\blacksquare$

\begin{corollary}
\label{corollary:monotonicity}
    Let $R_{\sigma_i} \coloneqq \log{R(\scdl;m,\sigma_i)}=(U(\scdl) - m)/ \sigma_i$ be a sequence of temperature conditioned reward functions with $\sigma_i \searrow \sigma_0$. Then, for any $\epsilon>0$ and flow $F^{R_{\sigma_0}}$ there exists a neighborhood  $(\sigma_0, \sigma_0+\delta)$ containing flow functions $F^{R_\sigma}$ with $F^{R_\sigma}(\trj)-F^{R_{\sigma_0}}(\trj) <\epsilon$ for all $\trj \in \mathcal{T}$. Furthermore, we can  approximate $F^{R_{\sigma_0}}$ with monotonically changing flow functions $F^{R_{\sigma_i}}$.
\end{corollary}
